ReasonAny: Incorporating Reasoning Capability to Any Model via Simple and Effective Model Merging

Large Reasoning Models (LRMs) with long chain-of-thought reasoning have recently achieved remarkable success. Yet, equipping domain-specialized models with such reasoning capabilities, referred to as "Reasoning + X", remains a significant challenge. While model merging offers a promising training-free solution, existing methods often suffer from a destructive performance collapse: existing methods tend to both weaken reasoning depth and compromise domain-specific utility. Interestingly, we identify a counter-intuitive phenomenon underlying this failure: reasoning ability predominantly resides in parameter regions with low gradient sensitivity, contrary to the common assumption that domain capabilities correspond to high-magnitude parameters. Motivated by this insight, we propose ReasonAny, a novel merging framework that resolves the reasoning-domain performance collapse through Contrastive Gradient Identification. Experiments across safety, biomedicine, and finance domains show that ReasonAny effectively synthesizes "Reasoning + X" capabilities, significantly outperforming state-of-the-art baselines while retaining robust reasoning performance.

==> latex/tables/hyperparameter_settings/hyperparameter_settings.tex <==
% \begin{table}[t!]
%     \centering
%     \renewcommand{\arraystretch}{1.5}
%     \small
%     \caption{Hyperparameter Setting of merging methods.}
%     \label{tab:hyperparameters}
%     \resizebox{\columnwidth}{!}{
%          \begin{tabular}{l|l}
%             \hline
%             \textbf{Model Merging Methods} &\textbf{Hyperparameter Settings} \\ 
%             \hline
%             \textbf{Task Arithmetic}&  \\
%             \hline
%             \textbf{TIES-Merging}&  \\
%             \hline
%             \textbf{DARE} &  \\
%             \hline
%             \textbf{FuseLLM} &  \\
%             \hline
%             \textbf{LED-Merging} &  \\
%             \hline
%             \textbf{ReasonAny (Ours)} &  \\
%             \hline
%         \end{tabular}
%     }
% \end{table}
